CCMR: High Resolution Optical Flow Estimation via Coarse-to-Fine Context-Guided Motion Reasoning

Attention-based motion aggregation concepts have recently shown their usefulness in optical flow estimation, in particular when it comes to handling occluded regions. However, due to their complexity, such concepts have been mainly restricted to coarse-resolution single-scale approaches that fail to provide the detailed outcome of high-resolution multi-scale networks. In this paper, we hence propose CCMR: a high-resolution coarse-to-fine approach that leverages attention-based motion grouping concepts to multi-scale optical flow estimation. CCMR relies on a hierarchical two-step attention-based context-motion grouping strategy that first computes global multi-scale context features and then uses them to guide the actual motion grouping. As we iterate both steps over all coarse-to-fine scales, we adapt cross covariance image transformers to allow for an efficient realization while maintaining scale-dependent properties. Experiments and ablations demonstrate that our efforts of combining multi-scale and attention-based concepts pay off. By providing highly detailed flow fields with strong improvements in both occluded and non-occluded regions, our CCMR approach not only outperforms both the corresponding single-scale attention-based and multi-scale attention-free baselines by up to 23.0% and 21.6%, respectively, it also achieves state-of-the-art results, ranking first on KITTI 2015 and second on MPI Sintel Clean and Final. Code and trained models are available at https://github.com/cv-stuttgart /CCMR.

==> encoder.tex <==
\begin{tikzpicture}
    \node [image] (image) {Image$_j$};
    \node [conv down, below=\DefaultDistance of image] (conv down) {conv\down};
    \node [residual unit, below=\DefaultDistance of conv down] (res 4) {res\vphantom{\down}};
    \node [residual unit, below=of res 4] (res 3) {res\down};
    \node [residual unit, below=of res 3] (res 2) {res\down};
    \node [residual unit, below=of res 2] (res 1) {res\down};

    \foreach \i in {2, 3, 4}
    {
        \node [intermediate feature, right=2*\DefaultDistance of res \i.south, yshift=-\BelowResOffset] (intermediate feature \i) {int-$f_{\i,j}$};
        \node [intermediate feature, right=\DefaultDistance of intermediate feature \i] (intermediate feature \i part) {};
        \node [feature, right=0pt of intermediate feature \i part] (upsampled intermediate feature \i part) {};
        \node [residual unit, right=\DefaultDistance of upsampled intermediate feature \i part] (new res \i) {res};
        \node [conv, right=\DefaultDistance of new res \i] (conv star \i) {conv\Star};
        \node [feature, right=\DefaultDistance of conv star \i] (feature \i) {$f_{\i,j}$};

        \draw[->] (res \i) |- (intermediate feature \i);
        \draw[->] (intermediate feature \i) -- (intermediate feature \i part);
        \draw[->] (upsampled intermediate feature \i part) -- (new res \i);
        \draw[->] (new res \i) -- (conv star \i);
        \draw[->] (conv star \i) -- (feature \i);
    }
    
    \node [conv, fill=res color, yshift=-\BelowResOffset] at (res 1.south -| conv star 2)  (conv star 1) {conv\Star};
    \node [feature, right=\DefaultDistance of conv star 1] (feature 1) {$f_{1,j}$};

    \draw[->] (image) -- (conv down);
    \draw[->] (conv down) -- (res 4);
    \draw[->] (res 4) -- (res 3);
    \draw[->] (res 3) -- (res 2);
    \draw[->] (res 2) -- (res 1);
    \draw[->] (res 1) |- (conv star 1);
    \draw[->] (conv star 1) -- (feature 1);

    \foreach \i/\j in {1/2, 2/3, 3/4}
    {
        \node[upsampler, yshift=-4pt] at ($(conv star \i)!0.5!(conv star \j)$) (upsampler \i \j) {\up};
        \draw[->] (feature \i) |- (upsampler \i \j) -| (upsampled intermediate feature \j part);
    }
    \foreach \i in {1, ..., 4}
    {
        \pgfmathsetmacro{\scaleDenominator}{int(pow(2, 5-\i))}
        \draw[brace] (feature \i.south east) -- (feature \i.south west) node[description, midway, below, yshift=-2pt] {$\frac{1}{\scaleDenominator} {\times} (h, w)$};
    }
\end{tikzpicture}


==> figures/feat_map.tex <==
    \begin{subfigure}[c]{0.95\columnwidth}%
     \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/temple2_frame_0019.png}
            %\vspace{-5mm}
            %\caption{}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/cave4_frame_0005.png}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}%
        \hfill%
         \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/market2_frame_0015.png}
            %\caption{CMAX+ (Ours)}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}
        \\%[1ex]
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/ohne/attn_0_norm.png}
            %\vspace{-5mm}
            %\caption{}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/ohne/attn_1_norm.png}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}%
        \hfill%
         \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/ohne/attn_2_norm.png}
            %\caption{CMAX+ (Ours)}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}
        \\%[1ex]
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/attn_0_norm.png}
            %\caption{FlowFormer}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/attn_1_norm.png}
            %\caption{SKFlow}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/attn_2_norm.png}
            %\caption{SKFlow}
        \end{subfigure}\\ 
    \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/foreground/attn_0_4_6.png}
            %\vspace{-5mm}
            %\caption{}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/foreground/attn_1_4_6.png}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}%
        \hfill%
         \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/foreground/attn_2_4_6.png}
            %\caption{CMAX+ (Ours)}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}
        \\
     \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/background/attn_0_5_15.png}
            %\vspace{-5mm}
            %\caption{}
        \end{subfigure}%
        \hfill%
        \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/background/attn_1_5_15.png}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}%
        \hfill%
         \begin{subfigure}{0.333\textwidth}
            \includegraphics[width=\textwidth]{feat_maps/mit/background/attn_2_5_15.png}
            %\caption{CMAX+ (Ours)}
            %\vspace{-5mm}
            %\caption{Ours}
        \end{subfigure}
    \end{subfigure}%
    %
    \hfill%
    \begin{subfigure}[c]{0.044\columnwidth}
        \vspace{0pt}
        \includegraphics[width=\textwidth]{figures/colorbar.pdf}%
    \end{subfigure}   


==> figures/kitti-test-15.tex <==
\NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
    \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
    \begin{scope}[x={(image.north east)}, y={(image.south west)}]
        \IfNoValueF{#2}{\node [anchor=south west, font=\tiny, inner sep=1pt] at (0, 1) {#2};}
    \end{scope}
\end{tikzpicture}}%
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/ours.png}[Fl-all 6.78]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/ours.png}
    \end{subfigure}
    \caption{CMAX+ (Ours)}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/raft-it+.png}[Fl-all 8.41]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/raft-it+.png}
    \end{subfigure}
    \caption{RAFT-it+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/raft-octc.png}[Fl-all 8.76]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/raft-octc.png}
    \end{subfigure}
    \caption{RAFT-OCTC}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/ms-raft+.png}[Fl-all 6.83]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/ms-raft+.png}
    \end{subfigure}
    \caption{MS-RAFT+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/kpa.png}[Fl-all 9.12]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/kpa.png}
    \end{subfigure}
    \caption{KPA-Flow}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-15/gmflow.png}[Fl-all 14.89]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-15/gmflow.png}
    \end{subfigure}
    \caption{GMFlow}
\end{subfigure}

==> figures/kitti-test-19.tex <==
\NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
    \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
    \begin{scope}[x={(image.north east)}, y={(image.south west)}]
        \IfNoValueF{#2}{\node [anchor=south west, font=\tiny, inner sep=1pt] at (0, 1) {#2};}
    \end{scope}
\end{tikzpicture}}%
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/ours.png}[Fl-all 2.07]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/ours.png}
    \end{subfigure}
    \caption{CMAX+ (Ours)}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/raft-it+.png}[Fl-all 3.48]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/raft-it+.png}
    \end{subfigure}
    \caption{RAFT-it+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/raft-octc.png}[Fl-all 3.41]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/raft-octc.png}
    \end{subfigure}
    \caption{RAFT-OCTC}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/ms-raft+.png}[Fl-all 2.10]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/ms-raft+.png}
    \end{subfigure}
    \caption{MS-RAFT+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/kpa.png}[Fl-all 3.80]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/kpa.png}
    \end{subfigure}
    \caption{KPA-Flow}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-19/gmflow.png}[Fl-all 13.19]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-19/gmflow.png}
    \end{subfigure}
    \caption{GMFlow}
\end{subfigure}

==> figures/kitti-test-8.tex <==
\NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
    \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
    \begin{scope}[x={(image.north east)}, y={(image.south west)}]
        \IfNoValueF{#2}{\node [anchor=south east, font=\tiny, fill=white, inner sep=1pt] at (1, 1) {#2};}
    \end{scope}
\end{tikzpicture}}%
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/ours.png}[Fl-all 0.46]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/ours.png}
    \end{subfigure}
    \caption{CMAX+ (Ours)}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/raft-it+.png}[Fl-all 0.58]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/raft-it+.png}
    \end{subfigure}
    \caption{RAFT-it+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/raft-octc.png}[Fl-all 0.63]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/raft-octc.png}
    \end{subfigure}
    \caption{RAFT-OCTC}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/ms-raft+.png}[Fl-all 0.68]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/ms-raft+.png}
    \end{subfigure}
    \caption{MS-RAFT+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/kpa.png}[Fl-all 0.65]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/kpa.png}
    \end{subfigure}
    \caption{KPA-Flow}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \centering
    \begin{subfigure}{0.49\textwidth}
        \flowimage{flows/test-8/gmflow.png}[Fl-all 0.46]
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \flowimage{errors/test-8/gmflow.png}
    \end{subfigure}
    \caption{GMFlow}
\end{subfigure}

==> figures/sintel-clean.tex <==
\NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
    \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
    \begin{scope}[x={(image.north east)}, y={(image.south west)}]
        \IfNoValueF{#2}{\node [anchor=south west, font=\tiny, inner sep=1pt] at (0, 1) {#2};}
    \end{scope}
\end{tikzpicture}}%
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/ours.png}[EPE 0.232]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/ours.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/ours.png}[EPE 0.297]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/ours.png}
    \end{subfigure}
    \caption{CMAX+ (Ours)}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/flowformer.png}[EPE 0.375]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/flowformer.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/flowformer.png}[EPE 0.439]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/flowformer.png}
    \end{subfigure}
    \caption{FlowFormer}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/skflow.png}[EPE 0.398]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/skflow.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/skflow.png}[EPE 0.478]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/skflow.png}
    \end{subfigure}
    \caption{SKFlow}
\end{subfigure}
\\[2pt]
%\begin{subfigure}{\textwidth}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{flows/temple-1/clean/kpa-flow.png}[EPE 0.403]
%    \end{subfigure}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{errors/temple-1/clean/kpa-flow.png}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{flows/tiger/clean/kpa-flow.png}[EPE 0.482]
%    \end{subfigure}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{errors/tiger/clean/kpa-flow.png}
%    \end{subfigure}
%    \caption{KPA-Flow}
%\end{subfigure}
%\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/gma.png}[EPE 0.489]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/gma.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/gma.png}[EPE 0.531]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/gma.png}
    \end{subfigure}
    \caption{GMA}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/ms-raft+.png}[EPE 0.313]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/ms-raft+.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/ms-raft+.png}[EPE 0.303]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/ms-raft+.png}
    \end{subfigure}
    \caption{MS-RAFT+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/dip.png}[EPE 0.619]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/dip.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/dip.png}[EPE 0.398]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/dip.png}
    \end{subfigure}
    \caption{DIP}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/temple-1/clean/gmflow.png}[EPE 0.641]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/temple-1/clean/gmflow.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/tiger/clean/gmflow.png}[EPE 0.602]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/tiger/clean/gmflow.png}
    \end{subfigure}
    \caption{GMFlow}
\end{subfigure}

==> figures/sintel-final.tex <==
% ours, flowformer, skflow, ms-raft+, gmflow, dip
% sintel final: bamboo, market 1
\NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
    \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
    \begin{scope}[x={(image.north east)}, y={(image.south west)}]
        \IfNoValueF{#2}{\node [anchor=south west, font=\tiny, inner sep=1pt] at (0, 1) {#2};}
    \end{scope}
\end{tikzpicture}}%
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/ours.png}[EPE 0.377]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/ours.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/ours.png}[EPE 0.913]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/ours.png}
    \end{subfigure}
    \caption{CMAX+ (Ours)}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/flowformer.png}[EPE 0.577]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/flowformer.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/flowformer.png}[EPE 1.174]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/flowformer.png}
    \end{subfigure}
    \caption{FlowFormer}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/skflow.png}[EPE 0.623]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/skflow.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/skflow.png}[EPE 1.045]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/skflow.png}
    \end{subfigure}
    \caption{SKFlow}
\end{subfigure}
\\[2pt]
%\begin{subfigure}{\textwidth}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{flows/bamboo-3/final/kpa-flow.png}[EPE 0.6124]
%    \end{subfigure}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{errors/bamboo-3/final/kpa-flow.png}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{flows/market-1/final/kpa-flow.png}[EPE 1.211]
%    \end{subfigure}
%    \begin{subfigure}{0.24\textwidth}
%        \flowimage{errors/market-1/final/kpa-flow.png}
%    \end{subfigure}
%    \caption{KPA-Flow}
%\end{subfigure}
% \\[2pt]
% \begin{subfigure}{\textwidth}
%     \begin{subfigure}{0.24\textwidth}
%         \flowimage{flows/bamboo-3/final/craft.png}[EPE 0.656]
%     \end{subfigure}
%     \begin{subfigure}{0.24\textwidth}
%         \flowimage{errors/bamboo-3/final/craft.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\textwidth}
%         \flowimage{flows/market-1/final/craft.png}[EPE 1.207]
%     \end{subfigure}
%     \begin{subfigure}{0.24\textwidth}
%         \flowimage{errors/market-1/final/craft.png}
%     \end{subfigure}
%     \caption{CRAFT}
% \end{subfigure}
%\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/gma.png}[EPE 0.649]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/gma.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/gma.png}[EPE 1.212]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/gma.png}
    \end{subfigure}
    \caption{GMA}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/ms-raft+.png}[EPE 0.407]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/ms-raft+.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/ms-raft+.png}[EPE 1.116]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/ms-raft+.png}
    \end{subfigure}
    \caption{MS-RAFT+}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/dip.png}[EPE 0.494]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/dip.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/dip.png}[EPE 1.263]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/dip.png}
    \end{subfigure}
    \caption{DIP}
\end{subfigure}
\\[2pt]
\begin{subfigure}{\textwidth}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/bamboo-3/final/gmflow.png}[EPE 0.740]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/bamboo-3/final/gmflow.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.24\textwidth}
        \flowimage{flows/market-1/final/gmflow.png}[EPE 1.223]
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \flowimage{errors/market-1/final/gmflow.png}
    \end{subfigure}
    \caption{GMFlow}
\end{subfigure}

==> figures/teaser.tex <==
    \NewDocumentCommand{\flowimage}{m o}{\begin{tikzpicture}
        \node [anchor=north west, inner sep=0pt] (image) at (0,0) {\includegraphics[width=\textwidth]{#1}};
        \begin{scope}[x={(image.north east)}, y={(image.south west)}]
            \draw [black, densely dotted] (0.24, 0.48) rectangle (0.27, 0.59);
            \draw [black, densely dotted] (0.37, 0.01) rectangle (0.57, 0.42);
            \draw [black, densely dotted] (0.43, 0.44) rectangle (0.67, 0.76);
            \IfNoValueF{#2}{\node [anchor=south west, font=\tiny, inner sep=1pt] at (0, 1) {#2};}
        \end{scope}
    \end{tikzpicture}}
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/groundtruth.png}
        \vspace{-5mm}
        \caption{Ground Truth}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/ours.png}[EPE 0.371]
        %\caption{CMAX+ (Ours)}
        \vspace{-5mm}
        \caption{Ours}
    \end{subfigure}
    \\%[1ex]
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/flowformer++.png}[EPE 0.511]
        \vspace{-5mm}
        \caption{FlowFormer++}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/gmflow+.png}[EPE 0.406]
        \vspace{-5mm}
        \caption{GMFlow+}
    \end{subfigure}
    \\%[1ex]
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/gma.png}[EPE 0.624]
        \vspace{-5mm}
        \caption{GMA}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
        \flowimage{flows/perturbed-market-3/clean/ms-raft+.png}[EPE 0.417]
        \vspace{-5mm}
        \caption{MS-RAFT+}
    \end{subfigure}
   

